Spectral-Timing Analysis of the Lower kHz QPO in the Low-Mass X-ray Binary Aquila X-1

Spectral-timing products of kilohertz quasi-periodic oscillations (kHz QPOs) in low-mass X-ray binary (LMXB) systems, including energy- and frequency-dependent lags, have been analyzed previously in 4U 1608-52, 4U 1636-53, and 4U 1728-34. Here, we study the spectral-timing properties of the lower kHz QPO of the neutron star LMXB Aquila X-1 for the first time. We compute broadband energy lags, as well as energy-dependent lags and the covariance spectrum using data from the Rossi X-ray Timing Explorer (RXTE). We find very similar characteristics to other previously studied systems, including soft lags of $\sim$30 $\mu$s between the 3.0 - 8.0 keV and 8.0 - 20.0 keV energy bands at the average QPO frequency. We also find lags that show a nearly monotonic trend with energy, with the highest energy photons arriving first. The covariance spectrum of the lower kHz QPO is well fit by a thermal Comptonization model, though we find a higher seed photon temperature compared to the mean spectrum, which was also seen in Peille et al., (2015), and indicates the possibility of a composite boundary layer emitting region. Lastly, we see in one set of observations, an Fe K component in the covariance spectrum at 2.4-$\sigma$ confidence which may raise questions about the role of reverberation in the production of lags.

==> defn.tex <==
%-*-LaTeX-*-
% Copied from gmorris
% Note that some of these call others, eg \kmps uses \km.

% journals
\newcommand{\apj}{ApJ}
\newcommand{\mnras}{MNRAS}
\newcommand{\nat}{Nature}
\newcommand{\physrevB}{Phys. Rev. B}
\newcommand{\araa}{ARA\&A}                % "Ann. Rev. Astron. Astrophys."
\newcommand{\aap}{A\&A}                   % "Astron. Astrophys."
\newcommand{\aaps}{A\&AS}                 % "Astron. Astrophys. Suppl. Ser."
\newcommand{\aj}{AJ}                      % "Astron. J."
\newcommand{\apjs}{ApJS}                  % "Astrophys. J. Suppl. Ser."
\newcommand{\pasp}{PASP}                  % "Publ. Astron. Soc. Pac."
\newcommand{\apjl}{ApJ}                   % letter at ApJ
\newcommand{\pasj}{PASJ}
\newcommand{\gca}{Geochim. Cosmochim. Acta}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\aapr}{AA\&AR}     % Astronomy and Astrophysics Review (the)}
\newcommand{\ssr}{Space Science Reviews}     % Astronomy and Astrophysics Review (the)}
\newcommand{\nar}{New Astronomy Reviews}


% Length
\newcommand{\Mpc}{\rm\thinspace Mpc}
\newcommand{\kpc}{\rm\thinspace kpc}
\newcommand{\pc}{\rm\thinspace pc}
\newcommand{\km}{\rm\thinspace km}
\newcommand{\m}{\rm\thinspace m}
\newcommand{\cm}{\rm\thinspace cm}
%
\newcommand{\cmps}{\hbox{$\cm\s^{-1}\,$}}
\newcommand{\cmpssq}{\hbox{$\cm\s^{-2}\,$}}
\newcommand{\cmsq}{\hbox{$\cm^2\,$}}
\newcommand{\cmcu}{\hbox{$\cm^3\,$}}
\newcommand{\pcmcu}{\hbox{$\cm^{-3}\,$}}
\newcommand{\pcmcuK}{\hbox{$\cm^{-3}\K\,$}}
% Length


% Time
\newcommand{\yr}{\rm\thinspace yr}
\newcommand{\Gyr}{\rm\thinspace Gyr}
\newcommand{\s}{\rm\thinspace s}
\newcommand{\ks}{\rm\thinspace ks}
% Time


% Frequency
\newcommand{\GHz}{\rm\thinspace GHz}
\newcommand{\MHz}{\rm\thinspace MHz}
\newcommand{\Hz}{\rm\thinspace Hz}
% Frequency


% Temperature
\newcommand{\K}{\rm\thinspace K}
% Temperature


% Pressure
\newcommand{\Kpcmc}{\hbox{$\K\cm^{-3}\,$}}
\newcommand{\keVpcmcu}{\hbox{$\keV\cm^{-3}\,$}}
% Pressure


% Mass
\newcommand{\g}{\rm\thinspace g}
%
\newcommand{\gpcm}{\hbox{$\g\cm^{-3}\,$}}
\newcommand{\gpcmps}{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\newcommand{\gps}{\hbox{$\g\s^{-1}\,$}}
%
\newcommand{\Msun}{\hbox{$\rm\thinspace M_{\odot}$}}
\newcommand{\Msunpc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunpkpc}{\hbox{$\Msun\kpc^{-1}\,$}}
\newcommand{\Msunppc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunppcpyr}{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\newcommand{\Msunpyr}{\hbox{$\Msun\yr^{-1}\,$}}
% Mass


% Energy
\newcommand{\MeV}{\rm\thinspace MeV}
\newcommand{\keV}{\rm\thinspace keV}
\newcommand{\eV}{\rm\thinspace eV}
\newcommand{\erg}{\rm\thinspace erg}
\newcommand{\Jy}{\rm Jy}
\newcommand{\photon}{\rm photon}
%
\newcommand{\ergcmcups}{\hbox{$\erg\cm^3\ps\,$}}
\newcommand{\ergpcmps}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergpcmsq}{\hbox{$\erg\cm^{-2}\,$}}
\newcommand{\ergpcmcu}{\hbox{$\erg\cm^{-3}\,$}}
\newcommand{\ergpcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergpcmsqpspA}{\hbox{$\erg\cm^{-2}\s^{-1}$\AA$^{-1}\,$}}
\newcommand{\ergpcmsqpspsr}{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\ergpcmcups}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergps}{\hbox{$\erg\s^{-1}\,$}}
\newcommand{\ergpspmp}{\hbox{$\erg\s^{-1}\Mpc^{-3}\,$}}
%
\newcommand{\keVpcmsqpspsr}{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\photoncmsqps}{\hbox{$\photon\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
% Energy


% Force
\newcommand{\dyn}{\rm\thinspace dyn}
\newcommand{\dynpcmsq}{\hbox{$\dyn\cm^{-2}\,$}}
% Force


% Speed
\newcommand{\kmps}{\hbox{$\km\s^{-1}\,$}}
\newcommand{\kmpspmp}{\hbox{$\km\s^{-1}\Mpc{-1}\,$}}
\newcommand{\kmpspMpc}{\hbox{$\kmps\Mpc^{-1}$}}
% Speed


% Luminosity
\newcommand{\Lsun}{\hbox{$\rm\thinspace L_{\odot}$}}
\newcommand{\Lsunppc}{\hbox{$\Lsun\pc^{-3}\,$}}
% Luminosity


% Misc
%\newcommand{\Zsun}{\hbox{$\rm\thinspace Z_{\odot}$}}
\newcommand{\Zsun}{\hbox{$\thinspace \mathrm{Z}_{\odot}$}}

\newcommand{\gauss}{\rm\thinspace gauss}
%
\newcommand{\chisq}{\hbox{$\chi^2$}}
\newcommand{\delchi}{\hbox{$\Delta\chi$}}
%
\newcommand{\ph}{\rm\thinspace ph}
\newcommand{\sr}{\rm\thinspace sr}
% Misc


% Per something
\newcommand{\pcm}{\hbox{$\cm^{-3}\,$}}
\newcommand{\psqcm}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmsq}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pmpc}{\hbox{$\Mpc^{-1}\,$}}
\newcommand{\pmpccu}{\hbox{$\Mpc^{-3}\,$}}
\newcommand{\ps}{\hbox{$\s^{-1}\,$}}
\newcommand{\pHz}{\hbox{$\Hz^{-1}\,$}}
\newcommand{\pcmK}{\hbox{$\cm^{-3}\K$}}
\newcommand{\phpcmsqps}{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\newcommand{\psr}{\hbox{$\sr^{-1}\,$}}
% Per something

\newcommand{\amin}{\rm\thinspace arcmin}
\newcommand{\aminsq}{\hbox{$\amin^{2}\,$}}
\newcommand{\asec}{\rm\thinspace arcsec}
\newcommand{\asecsq}{\hbox{$\asec^{2}\,$}}
\newcommand{\kpcsq}{\hbox{$\kpc^{2}\,$}}

% Use times for maths fonts
% \DeclareSymbolFont{operators}   {OT1}{ptmcm}{m}{n}
% \DeclareSymbolFont{letters}     {OML}{ptmcm}{m}{it}
% \SetMathAlphabet{\mathbf}{normal}{\encodingdefault}{\rmdefault}{\bfdefault}{n}%
% \SetMathAlphabet{\mathsf}{normal}{\encodingdefault}{\sfdefault}{m}{n}%
% \SetMathAlphabet{\mathrm}{normal}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetSymbolFont{operators}{bold}{OT1}{ptmcm}{b}{n}
% \SetSymbolFont{letters}{bold}{OML}{ptmcm}{b}{it}
% \SetMathAlphabet{\mathbf}{bold}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}%
% \SetMathAlphabet{\mathrm}{bold}{\encodingdefault}{\rmdefault}{b}{n}%

%\thinmuskip=2.5mu
%\medmuskip=3.5mu plus 1mu minus 1mu
%\thickmuskip=4.5mu plus 1.5mu minus 1mu
%\DeclareSymbolFont{symbols}     {OMS}{cmsy}{m}{n}
%\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
%\SetSymbolFont{symbols}{bold}{OMS}{cmsy}{b}{n}
%\SetSymbolFont{largesymbols}{bold}{OMX}{cmex}{m}{n}

